Lectures on Hausdorff and Gromov-Hausdorff Distance Geometry

The course was given at Peking University, Fall 2019. We discuss the following subjects: (1) Introduction to general topology, hyperspaces, metric and pseudometric spaces, graph theory. (2) Graphs in metric spaces, minimum spanning tree, Steiner minimal tree, Gromov minimal filling. (3) Hausdorff distance, Vietoris topology, Limits theory, inheritance of completeness, total boundedness, compactness by hyperspaces. (4) Gromov-Hausdorff distance, triangle inequality, positive definiteness for isometry classes of compact spaces, counterexample for boundedly compact spaces. (5) Gromov-Hausdorff distance for separable spaces in terms of their isometric images in \ell_\infty, correspondences, Gromov-Hausdorff distance in terms of correspondences. (6) Epsilon-isometries and Gromov-Hausdorff distance. (7) Irreducible correspondences and Gromov-Hausdorff distance. (8) Gromov-Hausdorff convergence, inheritance of metric and topological properties while Gromov-Hausdorff convergence. (9) Gromov-Hausdorff space (GH-space), optimal correspondences, existence of closed optimal correspondences for compact metric spaces, GH-space is geodesic. (10) Cover number, packing number, total boundedness, completeness, and separability of GH-space. (11) mst-spectrum in terms of GH-distances to simplexes, Steiner problem in GH-space. (12) GH-distance to simplexes with more points, GH-distance to simplexes with at most the same number of points. (13) Generalized Borsuk problem, solution of Generalized Borsuk problem in terms of GH-distances, clique covering number and chromatic number of simple graphs, their dualities, calculating these numbers in terms of GH-distances.

==> lt02-2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \chapter{Hausdorff distance. The case of Euclidean space.}
 \markboth{\chaptername~\thechapter.~Hausdorff distance. The case of Euclidean space.}%
          {\chaptername~\thechapter.~Hausdorff distance. The case of Euclidean space.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{plan}

\end{plan}

We return to the study of the geometry of the space $\cH (X)$ of closed bounded subsets of the metric space\-rank\-space $X$. According to the problem~\ref{prb:metric-simple-props}, for any nonempty $A\ss X$ the set $B_r (A)$ is a closed subset of $X$. It is clear that for bounded $A$ the set $B_r (A)$ is also bounded. Thus, the following proposition is proved.

\begin{prop}
For any metric space $X$, each $A\in\cH (X)$ and any non-negative $r$ we have $B_r (A)\in\cH (X)$.
\end{prop}

Recall also that, by the proposition~\ref{prop:HausdAttainsForComp}, the Hausdorff distance $d_H (A, B)$ is equal to the smallest $r$ for which $A\ss B_r (B)$ and $B\ss B_r (A)$.

We turn to the study of sets lying between arbitrary $A$ and $B$ from $\cH (X)$. For convenience, we introduce the following concept.

\begin{dfn}
Let $W$ be an arbitrary metric space, $a, b\in W$, $|ab|=r$, $s\in [0, r]$. We say that $c\in W$ is in the $s$ position between $a$ and $b$ if $|ac|=s$ and $|cb|=r-s$.
\end{dfn}

The following sentence follows directly from the sentence~\ref{prop:HausdAttainsForComp}.

\begin{prop}\label{prop:Cs-general}
Let $X$ be an arbitrary metric space and $A, B\in\cH (X)$, $r=d_H (A, B)$, $s\in [0, r]$. Then if the set $C\in\cH (X)$ is in the\emph{$s$ -position\/} between $A$ and $B$, then $C\ss B_s (A)\cap B_{rs} (B)$.
\end{prop}

\begin{notation}
The set $B_s (A)\cap B_{rs} (B)$ from the sentence~\ref{prop:Cs-general} will be denoted by $C_s (A, B)$ or, if it is clear, what $A$ and $B$ in question, then simply through $C_s$.
\end{notation}

\begin{rk}\label{rk:whenCsINcHX}
The set $C_s$ lies in $\cH (X)$ if and only if $C_s\ne\0$. An example of an empty $C_s$ is easy to build: take $X$, say $\R\sm\{0\}$, and put $A=\{- 1\}$, $B=\{1\}$ and $s=1$. It is easy to see that in this case $C_1=\0$.
\end{rk}

Let us give an example of a description of sets that are in the $s$ -position between some $A$ and $B$ from $\cH (X)$.

\begin{prop}\label{prop:one-point-sets}
Let $X$ be an arbitrary metric space and $A=\{a\}$, $B=\{b\}$, $r=|ab|$, $s\in [0, r]$. Then
\begin{enumerate}
\item $C_s$ is the set of all points from $X$ located between $a$ and $b$ in the $s$ position\/\rom;
\item $C_s$ is in the $s$ position between $A$ and $B$ if and only if $C_s\ne\0$\/\rom;
\item the set $C\in X$ is in the $s$ position between $A$ and $B$ if and only if $C$ is a nonempty closed subset of $C_s$.
\end{enumerate}
\end{prop}

\begin{proof}
The first statement is obvious.

To prove the second assertion, in addition to the remark~\ref{rk:whenCsINcHX}, it is also necessary to show that $C_s$ is in $s$ along the same ne. We only check $d_H (A, C_s)\le s$, since the inequality $d_H (B, C_s)\le r-s$ is proved in exactly the same way. Since $|Ac|=s$ holds for each $c\in C_s$, we have $C_s\ss B_s (A)$. Since $A$ is one-point, we also have $A\ss B_s (c)\ss B_s (C_s)$, as required.

Finally, we describe all $C\in\cH (X)$ located in $s$ along the same line between $A$ and $B$. At the suggestion of~\ref{prop:Cs-general}, each such $C$ is a nonempty closed subset of $C_s$. Conversely, if $C$ is a nonempty closed subset of $C_s$, then $C\in\cH (X)$ and for any $c\in C$ we have $A\ss B_s (c)\ss B_s (C )$ and, similarly, $B\ss B_{rs} (C)$, therefore $C$ is in the $s$ position between $A$ and $B$.
\end{proof}

\begin{rk}
In the sentence~\ref{prop:one-point-sets} we showed that for single-point $A$ and $B$ all sets $C$ located in the $s$ -position between $A$ and $B$ are are exactly all closed subsets of $C_s$. For non-point sets this is, generally speaking, not true. As an example, consider $A=[0,2]$ and $B=[3,5]$ on $X=\ R$, then $d_H (A, B)=3$. Take $s=1.5$, then $C_s=[1.5,3.5]$. Let $C=\{2.5\}\in C_s$. Then $d_H (A, C)=d_H (B, C)=2.5$, so $d_H (A, C)+d_H (B, C)> d_H (A, B)$.
\end{rk}

\begin{rk}
If in the previous example we take an arbitrary closed subset $C$ of the segment $C_s=[1.5,3.5]$ containing the boundary $\d C_s=\{1.5,3.5\}$ of this segment, we get $d_H (A, C)=d_H (B, C)=1.5=s$. This demonstrates that
in the $s$ -position between the data $A$ and $B$ there can be more than one (even infinitely many) sets $C\in\cH (X)$.
\end{rk}

The following theorem is proved in~\cite{Bogdewicz5} for the case $X=\R^n$.

\begin{thm}\label{thm:between_A_and_B}
Let $X$ be a complete locally compact space with intrinsic metric. Then for any $A,\, B\in\cH (X)$, $r=d_H (A, B)$, $s\in [0, r]$, the set $C_s=C_s (A, B)$ belongs to $\cH (X)$ and is in the $s$ position between $A$ and $B$.
\end{thm}

\begin{prb}
Give an example of a metric space $X$ and subsets $A, B\in\cH (X)$ for which some set $C_s$ does not lie in $\cH (X)$. Give an example where $C_s\in\cH (X)$, but $C_s$ is not in the $s$ position between $A$ and $B$.
\end{prb}

\begin{proof} [Proof of the theorem~$\ref {thm:between_A_and_B}$]
By the theorem~\ref{thm:Hopf-Rinow: 1}, the space $X$ is boundedly compact. In particular, the set $\cH (X)$ consists of all nonempty compact subsets of $X$. By the corollary~\ref{cor:LocalCompactInnerCompleteIsStrictlyInner}, the metric of the space $X$ is strictly internal.

Let us show that the set $C_s$ is nonempty. By the definition of the Hausdorff distance, for each point $a\in A$ we have $|aB|\le r$, and since $B$ is compact, there exists $b\in B$ for which $|ab|=|aB|$. Since the metric is strictly intrinsic, there exists a curve $\g (t)$, $t\in [0,1]$ for which $\g (0)= a$, $\g (1)=b$ and $|ab|=|\g|\le r$. Since the function $f (t)=\bigl|a\g (t)\bigr|$ is continuous, $f (0)=0$ and $f (1)\le r$, there exists $t_0$ such that $\bigl|a\g (t_0)\bigr|\le s$ and $\bigl|b\g (t_0)\bigr|\le rs$. Therefore, $\g (t_0)\in C_s$ and, therefore, $C_s\ne\0$. By virtue of the remark~\ref{rk:whenCsINcHX}, $C_s\in\cH (X)$.

We show now that $d_H (A, C_s)=s$ and $d_H (B, C_s)=r-s$. To do this, it suffices to verify that $d_H (A, C_s)\le s$ and $d_H (B, C_s)\le r-s$, since $d_H (A, B)=r$ and $d_H$ satisfy the triangle inequality. Let us prove that $d_H (A, C_s)\le s$ (the second inequality is obtained in exactly the same way).

Since $C_s\ss B_s (A)$, it suffices to verify that $A\ss B_s (C_s)$. As shown above, for each point $a\in A$ there exists a shortest curve $\g (t)$ coming out of $a$ such that for some of its point $\g (t_0)$ $\bigl|a\g (t_0)\bigr|\le s$ and $\g (t_0)\in C_s$. Therefore, $A\ss B_s (C_s)$, as required.
\end{proof}

\begin{cor}\label{cor:cHforBoundCompactStrictInner}
Let $X$ be a complete locally compact space with intrinsic metric\/\(=boundedly compact space with strictly intrinsic metric\). Then $\cH (X)$ is also boundedly compact, and the Hausdorff metric is strictly intrinsic.
\end{cor}

\begin{proof}
This follows from the theorems~\ref{thm:Hausdorff-compactness} and~\ref{thm:MiddlePoints}.
\end{proof}

In fact, the fact that the metric of the space $\cH (X)$ from the corollary~\ref{cor:cHforBoundCompactStrictInner} is strictly intrinsic can be proved explicitly by presenting for each pair of points in the space $\cH (X)$ the shortest path connecting them a curve.

\begin{cor}
Let $X$ be a complete locally compact space with an intrinsic metric, $A, B\in\cH (X)$, and $r=d_H (A, B)$. Then $\g (s)=C_s (A, B)$, $s\in [a, b]$, is the shortest curve connecting $A$ and $B$, and the length of the curve $\g$ is $d_H (A, B)$, and the parameter $s$ is natural.
\end{cor}

\begin{proof}
Consider $0\le t<s\le r$, then $d_H(A,C_t)=t$, $d_H(C_t,B)=rt$, $d_H(A,C_s)=s$, $d_H(C_s,B)=rs$. We show that $d_H(C_t,C_s)=s-t$, which completes the proof. Since, by virtue of the corollary~\ref{cor:cHforBoundCompactStrictInner}, the metric of the space $\cH (X)$ is strictly internal, the point $C_t$ is connected with $A$ and $B$ by the shortest curves $\dl_A$ and $\dl_B$ respectively, which together give the shortest curve $\dl^t$ connecting $A$ and $B$. On $\dl^t$ we choose the natural parameter $u\in[0,r]$, $\dl^t(0)=A$, $\dl^t(r)=B$, then $\dl^t(s)$ is in the $s$ position between $A$ and $B$. At the suggestion of~\ref{prop:Cs-general}, we have $\dl^t(s)\ss C_s$. Since $d_H\bigl(C_t,\dl^t(s)\bigr)=st$, then $C_t\ss B_{st}\bigl(\dl^t(s)\bigr)$ and, moreover, $C_t\ss B_{st} (C_s)$. We similarly show that $C_s\ss B_{s-t}(C_t)$, but then $d_{H}(C_t, C_s)\le s-t$. However, by the inequality of the triangle, we have
$$
d_H(C_t,C_s)\ge d_H(A,B)-d_H(A,C_t)-d_H(C_s,B)=r-t-(r-s)=s-t,
$$
whence $d_{H}(C_t,C_s)=s-t$, as required.
\end{proof}

\begin{thm}\label{thm:Cs_with_nonempty_interior}
Let $X$ be a complete locally compact space with internal metric and $A, B\in\cH (X)$, $r=d_H (A, B)> 0$, $s\in (0, r)$, $0 <\e\le\min\{s,\, rs\}/2$. Suppose that for some point $p\in C_s$, $U_\e (p)\ss C_s$ holds. Then $C_s\sm U_\e (p)$ is in the $s$ position between $A$ and $B$.
\end{thm}

\begin{proof}
As in the proof of the theorem~\ref{thm:between_A_and_B}, we conclude that $X$ is a boundedly compact space with a strictly internal metric.

Put $D=C_s\sm U_\e (p)$. Note that $D$ is a closed bounded set. Let us show that $D\ne\0$. Since $A\ne B$, without loss of generality, we can assume that $B\not\ss B_s (A)$, so there is $b\in B$, $b\not\in C_s$, so $|bC_s|> 0$ and, therefore, $|pb|>\e$. Let $\g (t)$, $t\in [0,1]$, be the shortest curve for which $\g (0)=p$ and $\g (1)=b$. In view of the above, we have $|\g|>\e$, therefore there is only $t_0$ for which $\bigl|p\g (t_0)\bigr|=\e$. It is clear that $\g (t_0)$ is the touch point of $U_\e (p)$ and, therefore, because $C_s$ is closed, we have $\g (t_0)\in C_s$. On the other hand, $\g (t_0)\not\in U_\e (p)$, so $\g (t_0)\in D$. Thus, we have proved that $D\in\cH (X)$.

Let us prove now that $D$ is in the $s$ position between $A$ and $B$. As in the proof of the theorem~\ref{thm:between_A_and_B}, we restrict ourselves to verifying that $A\ss B_s (D)$. Choose an arbitrary $a\in A$ and prove that $a\in B_s (D)$. By the theorem~\ref{thm: between_A_and_B}, we have $A\ss B_s (C_s)$, therefore $|aC_s|\le s$ and, due to the compactness of $C_s$, there exists $c\in C_s$ for which $|ac|\le s$. If $c\in D$, then $a\in B_s (D)$ and everything is proved.

Now let $c\in U_\e (p)$. If $a\in U_\e (p)$, then for the point $\g (t_0)\in D$ constructed above, we have $\bigl|a\g (t_0)\bigr|\le|ap|+\bigl|p\g (t_0)\bigr|<2\e\le s$, so $a\in B_s (D)$. If $a\not\in U_\e (p)$, then denote by $\g$ the shortest curve connecting $a$ and $c$. Then there exists $\g (t_0)$ for which $\bigl|p\g (t_0)\bigr|=\e$, so $\g (t_0)\in D$ and $\bigl|a\g (t_0)\bigr|<|ac|\le s$, whence again $a\in B_s (D)$.
\end{proof}

\begin{cor}\label{cor:Cs_with_nonempty_interior}
Let $X$ be a complete locally compact space with internal metric and $A, B\in\cH (X)$, $r=d_H (A, B)> 0$, $s\in (0, r)$. Suppose that the interior of the set $C_s$ is nonempty. Then there are infinitely many $C\in\cH (X)$ that are in the $s$ -position between $A$ and $B$.
\end{cor}

\begin{proof}
By the theorem~\ref{thm:Cs_with_nonempty_interior}, there are $p\in C_s$ and $\e> 0$ such that $U_\e (p)\ss C_s$ and $D_\e=C_s\sm U_\e (p)$ is in the $s$ position between $A$ and $B$. As was shown in the proof of the theorem~\ref{thm:Cs_with_nonempty_interior}, for the chosen $p$ and $\e$ there exists a point $x\in X$ such that $x\not\in U_\e (p)$ ( in the proof this point turned out to be $b\in B$). Again, choose the shortest curve $\g (t)$ connecting $p$ and $x$, and notice that for every $0 <\e_1 <\e_2\le\e$ there is $t_0$ for which $\g ( t_0)\in U_{\e_2} (p)\sm U_{\e_1} (p)$, i.e.\. all $U_\e (p)$, and with them all $D_\e$, are different.
\end{proof}

\begin{examp}
Even if the sets $A$ and $B$ are finite, there can still be an infinite number of sets between them in the $s$ -position. The simplest example is the two-point subset $A=\{0,3\}$ of the real line and the one-point $B=\{1\}$. Then $d_H (A, B)=2$ and for $s=1$ we have $C_s=[0,1]\cup\{2\}$, so that any closed $C\ss C_s$ containing $\{0,1,2\}$, is in the $s$ position between $A$ and $B$. There are infinitely many such $C$. In the corollary below, we find out another reason why there can be infinitely many sets in the $s$ -position.
\end{examp}

\begin{cor}\label{cor:When_A_and_B_have_infinitely_many_in_the_same_location}
Let $X$ be a complete locally compact space with an intrinsic metric and $A, B\in\cH (X)$, $r=d_H (A, B)> 0$. Suppose that there are $a\in A$ and $b\in B$ for which $|ab|<r$. Then for every $0 <s <r$ there are infinitely many $C\in\cH (X)$ that are in the $s$ -position between $A$ and $B$.
\end{cor}

\begin{proof}
Put $U=U_s (a)\cap U_{r-s} (b)$ and notice that $U\ss C_s$. Since the metric is strictly intrinsic, the set $U$ is nonempty (check), therefore $C_s$ has a nonempty interior and the corollary~\ref{cor:Cs_with_nonempty_interior} applies.
\end{proof}

In the two corollaries below, $X$ denotes a complete locally compact space with an intrinsic metric. Both results directly follow from the corollary~\ref{cor:When_A_and_B_have_infinitely_many_in_the_same_location}.

\begin{cor}
Suppose that for $A\ne B\in\cH (X)$, $r=d_H (A, B)$ and some $s\in (0, r)$ there is only a finite number of elements $C\in\cH (X)$ located in $s$ along the same line between $A$ and $B$. Then for any $a\in A$ and $b\in B$ we have $|ab|\ge r$.
\end{cor}

\begin{cor}\label{cor:finite_number_between}
Suppose that for $A\ne B\in\cH (X)$, $r=d_H (A, B)$ and some $s\in (0, r)$ there is only a finite number of elements $C\in\cH (X)$ located in $s$ along the same line between $A$ and $B$. Then for any $a\in A$ and $b\in B$ we have $|aB|=|Ab|=r$.
\end{cor}

Let $X$ be an arbitrary metric space. A pair of $\{A, B\}$ different sets from $\cH (X)$, $r=d_H (A, B)$, is called\emph{configuration} if for any $a\in A$ and $b\in B$, we have $|ab|\ge r$ (equivalent condition: if for any $a\in A$ and $b\in B$ we have $|aB|=|Ab|=r$). The configuration $\{A, B\}$ is called\emph{finite} if $A$ and $B$ have a finite number of elements, otherwise the configuration $\{A, B\}$ is called\emph{infinite}.

For the future it will also be convenient to introduce the following notation. Let $A$ and $B$ be an arbitrary pair of sets from $\cH (X)$. For each real $s$, denote by $N_s (A, B)$ the number of different sets from $\cH (X)$ between $A$ and $B$ in the $s$ -position. Note that if $r=d_H (A, B)$, then for $s\ not\in [0, r]$ we have $N_s (A, B)=0$. In addition, $N_0 (A, B)=N_r (A, B)=1$. For the remaining $s\in (0, r)$, the number $N_s (A, B)$ can be either finite or equal to $\infty$. Below we will study the properties of the function $N_s (A, B)$.

\begin{rk}
We note the following obvious property. Let $A$ and $B$ be arbitrary nonempty finite subsets of the metric space $X$, $r=d_H (A, B)> 0$, $s\in [0, r]$, then $C_s (A , B)=\cup_{a\in A,\, b\in B}\bigl (B_s (a)\cap B_{rs} (b)\bigr)$. It follows that if for any $x, y\in X$ and any $s\in\bigl [0,|xy|\bigr]$ the intersection is $B_s (x)\cap B_{|xy|-s} ( y)$ consists of a finite number of points, then for each finite configuration $\{A, B\}$ we have $N_s (A, B) <\infty$. In particular, this holds for the Euclidean space $X$. Moreover, in the case of Euclidean space and single-point $A=\{a\}$ and $B=\{b\}$ we have $N_s (A, B)=1$ for all $s\in\bigl [0,|ab|\bigr]$.
\end{rk}

\begin{examp}\label{examp:2k-angle-config}
On the Euclidean plane, consider a regular $2k$ -coal\-nick with side $1$, and let $A$ be the set of vertices of this polygon taken through one, and $B$ the set of remaining vertices. Then $d_H (A, B)=1$, and for every $s\in (0,1)$ the set $C_s$ consists of $2k$ points $c_1,\ldots, c_{2k}$ (we number these points sequentially at one of two rounds of the polygon). It is easy to see that there is more than one set $C$ located between $A$ and $B$ in the $s$ position, for example, $C=C_s\sm\{c_i\}$, or $C=C_s\sm\{c_1, c_3,\ldots, c_{2k-1}\}$.

\begin{prb}
Prove that for $s\in (0,1)$ and $k=3$ in the example~\ref{examp:2k-angle-config} $N_s (A, B)=18$ is executed. Calculate $N_s (A, B)$ for the remaining $k$.
\end{prb}

\begin{sol}
It is clear that $C_s$ consists of $2k$ points; moreover, for the condition $A\ss B_s (C)$ and $B\ss B {rs} (C)$ to be fulfilled, it is necessary and sufficient that for each vertex of the polygon at least on one of the edges adjacent to this vertex was a point from $C$. Consider only the edges of the original polygon that do not contain points from $C$. It follows from the above that in the obtained family no two edges are adjacent, and any family in which there are no adjacent edges is suitable. Such families are called\emph{matching\/} in the graph under consideration (representing the cycle $C_{2k}$). There is a whole science devoted to calculating the number of matching, see\. works of H.~Hosoya (for example~\cite{Hosoya5}), I.~Gutman (for example~\cite{Gutman5}), etc. Characteristic polynomials can be used to solve this problem.

Consider an arbitrary graph $G$ with $m$ edges, and let $p (G, i)$ denote the number of matchings in the graph $G$ consisting of $i$ edges. We construct the characteristic polynomial $Q_G (x)=\sum_{i=1}^mp (G, i) x^i$. Then the required number of combinations is $QG (1)$. It turns out that another polynomial is more convenient for calculations, namely,
$$
P_G (x)=x^mQ_G (-1/x^2)=\sum_{i=1}^m (-1)^ip (G, i) x^{m-2i}.
$$
It is interesting in that it can sometimes be calculated iteratively. For example, $P_G (C_m)=x\, P_G (C_{m-1}) - P_G (C_{m-2})$.~\cite{Hosoya5} calculated $P_{C_m} (x)$ for all $m$. Here is its specific view:
$$
P_{C_m} (x)=\sum_{i=0}^{[m/2]} (- 1)^i\frac m {m-i} C_{m-i}^ix^{m-2i}.
$$
In particular, $P_{C_6} (x)=x^6-6x^4+9x^2-2$, whence $Q_{C_6} (x)=2x^6+9x^4+6x^2+1$, so the desired number is $Q_{C_6} (1)=18$. However, it is equal to $P_{C_6} (- 1)$.
\end{sol}
\end{examp}

Note that finiteness of the number of sets in the $s$ -position can arise not only for finite configurations, but also for infinite ones.

\begin{examp} [Infinite configuration with a single set in each fixed position]\label{examp:infinite_config_with_unique_s_position}
Let $A$ and $B$ be two non-coincident concentric circles of radii $r_A> r_B$ respectively on the Euclidean plane. Then $r=d_H (A, B)=r_A-r_B$, and for every $s\in [0, r]$ the set $C_s$ is a circle concentric with $A$ and $B$ and having a radius $r_A-s$. Let $C$ be an arbitrary closed subset of $C_s$ that does not coincide with $C_s$. Then in $C_s$ there exists a point $x$ that does not belong to $C$ and, since $C$ is closed, is not a touch point for $C$, that is,\. for some $\e> 0$, $|xC|>\e$ holds. But then $A$ is not contained in $B_{s+\dl} (C)$ for sufficiently small $\dl$, so $d_H (A, C)> s$. Thus, in the above example, for every $s$ we have $N_s (A, B)=1$.

\begin{prb}
Find out when for two segments $A$ and $B$ on the Euclidean plane, $r=d_H (A, B)$, for every $s\in [0, r]$, $N_s (A, B)=1$. A similar question about $N_s (A, B) <\infty$.
\end{prb}

\begin{sol}
Let's start with the second task. By the corollary~\ref{cor:finite_number_between}, for any point $a\in A$ we have $|aB|=r$. The set of all points $x\in R^n$ located from the segment $B$ at the same distance $r$ is a straight circular cylinder with the axis of rotation $B$ (obtained by rotating around $B$ some segment $I$ obtained from $B$ by displacement by $r$ in any direction perpendicular to $B$), together with two `` caps''hemispheres. It follows from the above that the segment $A$ lies in the set just described, therefore it is contained in one of the segments $\v I$, where $\v$ is some rotation around $B$. Thus, the segment $A$ is no longer than $B$. It is similarly shown that $B$ is no longer than $A$, therefore these segments are equal in length, and, therefore, one of them is obtained from the second by a shift in a direction perpendicular to the other segment. It remains to note that for such segments $C_s$ there is also a segment obtained from $A$ by parallel translation over the distance $s$ in the direction of the vector connecting the midpoints of $A$ and $B$, moreover, if $C\ne C_s$ , then $A\not\ss B_s (C)$. Thus, if $N_s (A, B) <\infty$ for all $s$, then for all $s\in [0, r]$ we have $N_s (A, B)= 1$.
\end{sol}
\end{examp}

Let us give an example of an infinite configuration $\{A, B\}$ for which $N_s (A, B)=\infty$. Thus, the condition that the pair forms a configuration is not sufficient for finiteness of the number of intermediate sets in the same position.

\begin{examp}
Let $A$ be a subset of the Euclidean plane consisting of a circle of radius $2$ and its center, and $B$ a circle with the same center but radius $1$. Then $d_H (A, B)=1$, and for every $s\in (0,1)$ the set $C_s$ consists of two circles $C'$ and$ C''$. Let $C'$ be the smaller of these circles, and$ x $be its arbitrary point. Then each set$ C=C''\cup\{x\} $is contained in$\cH (\R^2) $and is in the$ s $-position between$ A $and$ B $.
\end{examp}

The following result, however, in a slightly different formulation and with a rather strange proof, can be found in~\cite{Honigs5}.

\begin{thm}\label{thm:const_N_s}
Let $X$ be a boundedly compact space with strictly intrinsic metric. Suppose further that any two points are connected by a unique shortest curve, up to parametrization, and that the shortest curves containing a common non-degenerate fragment lie in the same shortest curve. Let $\{A, B\}$ be an arbitrary configuration and $r=d_H (A, B)> 0$. Then the function $f (s)=N_s (A, B)$ is constant on $(0, r)$.
\end{thm}

\begin{proof}
We need the following auxiliary results.

\begin{lem}
Let $W$ be an arbitrary metric space, $K\ss W$ be some nonempty compact, and $r\ge 0$. Then $B_r (K)=\cup_{x\in K} B_r (x)$.
\end{lem}

\begin{proof}
It is clear that $\cup_{x\in K} B_r (x)\ss B_r (K)$. Let us prove the reverse inclusion.

Let $w$ be an arbitrary point from $B_r (K)$, then, by definition, $|wK|\le r$. Since $K$ is compact, there exists $x\in K$ such that $|wK|=|wx|$, whence $w\in B_r (x)$, which completes the proof.
\end{proof}

\begin{cor}\label{cor:Cs-cupcap}
Let $W$ be an arbitrary metric space, $K$ and $L$ be arbitrary nonempty compact subsets of $W$, and $r=d_H (K, L)$. Then for any $s\in [0, r]$
$$
C_s (K, L)=\mathop{\bigcup}\limits_{x\in K,\, y\in L}\bigl (B_s (x)\cap B_{r-s} (y)\bigr).
$$
\end{cor}

\begin{lem}\label{lem:uniquenessOfballsIntersection}
Let $W$ be an arbitrary space with strictly intrinsic metric. Then each pair of points $x$ and $y$ is connected by a unique shortest curve, up to a parameter change, if and only if for any $x, y\in X$, $r=|xy|$, and any $s\in [0, r]$ the set $B_s (x)\cap B_{rs} (y)$ consists of exactly one point.
\end{lem}

\begin{proof}
Assume first that each pair of points in $W$ is connected by a single shortest curve. Connect $x$ and $y$ of the naturally parameterized shortest curve $\g (t)$, $t\in [0, r]$, $\g (0)=x$, $\g (r)=y$ then for $p=\g (s)$ we have $p\in B_s (x)\cap B_{rs} (y)$, so the set $B_s (x)\cap B_{rs} (y)$ not empty. Moreover, all points of the curve $\g$ other than $p$ do not lie in $B_s (x)\cap B_{r-s} (y)$.
Suppose that the set $B_s (x)\cap B_{r-s} (y)$ contains some point $q\ne p$. Let $\g_1$ and $\g_2$ denote the shortest curves connecting $q$ with $x$ and $y$, respectively. We make suitable parameter changes on the curves $\g_i$ and consider gluing $\dl$ of the resulting curves. Then $|\dl|=|\g_1|+|\g_2|=|xq|+|qy|=|xy|$, so $\dl$ is also the shortest curve. It follows from the above that $\g$ and $\dl$ cannot be obtained from each other by changing the parameter, a contradiction.

Now let each set $B_s (x)\cap B_{r-s} (y)$ consist of exactly one point. We show that each pair of points in the space $W$ is connected by a unique shortest curve, up to parametrization. Assume the contrary, i.e.,\. that for some points $x$ and $y$ there are at least two shortest curves $\g$ and $\dl$ that cannot be obtained from each other by changing the parameter and connecting $x$ with $y$. We parameterize these curves with the natural parameter $t\in [0, r]$ so that $\g (0)=\dl (0)=x$ and $\g (r)=\dl (r)=y$. Then there exists $s\in [0, r]$ such that $\g (s)\ne\dl (s)$. Since $\g (s)$ and $\dl (s)$ are the only intersection points of these curves with the set $B_s (x)\cap B_{rs} (y)$, this set consists of more than one point, a contradiction.
\end{proof}

We apply the corollary~\ref{cor:Cs-cupcap} and the lemma~\ref{lem:uniquenessOfballsIntersection} to the configuration $\{A, B\}$. Since for all $a\in A$ and $b\in B$ we have $|ab|\ge r$, each set $C_s (a, b):=B_s (a)\cap B_{rs} ( b)$ is either empty (for $|ab|> r$), or, by the lemma~\ref{lem:uniquenessOfballsIntersection}, consists of one point (for $|ab|=r$), which we denote by $c_s (a, b)$. Thus, the set $C_s (a, b)$ is empty (nonempty) for some $s$ if and only if it is empty (respectively, nonempty) for any $s\in [0, r]$.

Next, denote by $M$ the set of all pairs $(a, b)$ for which $|ab|=r$, and define the mappings $\mu_s\: M\to C_s$ by setting $\mu_s\:( a , b)\mapsto c_s (a, b)$. By the lemma~\ref{cor:Cs-cupcap}, we have $C_s=\cup_{(a, b)\in M} C_s (a, b)$, so all the mappings $\mu_s$ are surjections. Let us show that all $\ mu_s$ for $s\in (0, r)$ is injective.

\begin{lem}\label{lem:mu_s_is_injection}
Let $(a_1, b_1)$ and $(a_2, b_2)$ be two different elements from $M$, then $c_s (a_1, b_1)\ne c_s (a_2, b_2)$ for every $s\in (0, r)$.
\end{lem}

\begin{proof}
Suppose this is not the case. Then the naturally parameterized shortest curves $\g_1 (t)$ and $\g_2 (t)$, $t\in [0, r]$, $\g_i (0)=a_i$, $\g_i (r)=b_i$, $i=1,\, 2$, intersect at some point $p=c_s (a_1, b_1)=c_s (a_2, b_2)=\g_1 (s)=\g_2 (s)$, but do not match. We denote the part of the curve $\g_i$ from $a_i$ to $p$ by $\g_{ia}$, and from $p$ to $b_i$ by $\g_{ib}$. Since $|\g_{1a}|=|\g_{2a}|=s$ and $|\g_{1b}|=|\g_{2b}|=rs$, we have $|\g_{ia}|+|\g_{jb}|=r$ for all $1\le i,\, j\le 2$. Since $\{A, B\}$ is a configuration, it follows that $|a_ib_j|\ge r$, therefore gluing together the curves $\g_{ia}$ and $\g_{jb}$ are the shortest curves.

Without loss of generality, suppose that $b_1\ne b_2$, then the gluings $\g_{1a}\cdot\g_{1b}=\g_1$ and $\g_{1a}\cdot\g_{2b}$ are different shortest curves containing a common non-degenerate fragment $\g_{1a}$, a contradiction.
\end{proof}

The lemma~\ref{lem:mu_s_is_injection}, together with the remark made above, prove that for every $s\in (0, r)$ the map $\mu_s$ is a bijection. In particular, all the sets $C_s$, $s\in (0, r)$, are equally powerful and have the same power as the set $M$.

\begin{lem}\label{lem:exactness_of_mu}
Let $s\in (0, r)$ and $c\in C_s$. Put $\mu_s^{- 1} (c)=\{(a, b)\}$. Then $B_s (c)\cap A=\{a\}$ and $B_{r-s} (c)\cap B=\{b\}$.
\end{lem}

\begin{proof}
Suppose the contrary. Without loss of generality, we assume that $B_s (c)\cap A$ contains $a'\ne a$. But then $|a'b|\le|a'c|+|cb|\le r$. On the other hand, since $\{A, B\}$ is a configuration, we have $|a'b|\ge r$, whence $|a'b|=r$, therefore $(a', b )\in M ??$ and$ c=\mu_s (a', b)=\mu_s (a, b) $, a contradiction with the lemma~\ref{lem:mu_s_is_injection}.
\end{proof}

To complete the proof of the theorem, we find out which of the subsets $C$ of the set $C_s$ are located between $A$ and $B$. Since $C\ss B_s (A)$ and $C\ss B_{rs} (B)$, $C$ is between $A$ and $B$ if and only if $A\ss B_s (C )$ and $B\ss B_{rs} (C)$, i.e.\. if for every point from $a\in A$ there exists $c\in C$ such that $a\in B_s (c)$ (similarly, for points from $B$).

Denote by $\pi_A$ the natural projection of the set $M$ onto $A$, that is,\. $\pi_A\:( a, b)\mapsto a$; similarly, let $\pi_B$ denote the natural projection of the set $M$ onto $B$. By the lemma~\ref{lem:exactness_of_mu}, for each $c\in C_s$ we have $B_s (c)\cap A=\pi_A\bigl (\mu_s^{- 1} (c)\bigr)$, therefore the fact that for every point in $a\in A$ there exists $c\in C$ for which $a\in B_s (c)$ is equivalent to the condition $\pi_A\bigl (\mu_s^{- 1} ( C)\bigr)=A$, i.e.\. surjectivity of the restriction of the projection of $\pi_A$ onto $\mu_s^{- 1} (C)$. Similarly, the corresponding condition for $B$ is equivalent to the surjectivity of the restriction of the projection $\pi_B$ onto $\mu_s^{- 1} (C)$. So, the number of $N_s (A, B)$ different $C\ss C_s$ located in $s$ position between $A$ and $B$ is equal to the number of subsets of the set $M$ whose projections onto $A$ and $B$ is surjective. But the last condition does not depend on $s$.
\end{proof}

Based on the theorem~\ref{thm:const_N_s}, for each finite configuration $\{A, B\}$ in a boundedly compact space with a strictly internal metric, we define the value $N (A, B)$ equal to $N_s (A, B )$ for an arbitrary $s\in\bigl (0, d_H (A, B)\bigr)$. A natural question arises: what can the numbers $N (A, B)$ be equal to? There is an amazing theorem proved in~\cite{Honigs5} and having applications in graph theory.

\begin{thm}\label{thm:19}
For every natural number $m$, $1\le m\le 37$, except for $m=19$ and $m=19$, there exists a finite configuration $\{A, B\}$ in some $\R^n$ for which $N (A, B)=m$. There is no finite or infinite configuration in $\R^n$ for which $N (A, B)=19$ and $N (A, B)=37$.
\end{thm}

It turns out that the theorem~\ref{thm:19} leads to a nontrivial result of graph theory. If $\{A, B\}$ is some configuration, $r=d_H (A, B)$, and $M$, as above, is the set of all pairs $(a, b)$, $a\in A$, $b\in B$ such that $|ab|=r$, then we put $V=A\cup B$ and $E=M$, then $G (A, B) :=(V, E)$ is a simple bipartite directed graph, which we will call\emph{configuration graph $\{A, B\}$}. It is clear that the graph $G (A, B)$ is finite if and only if the configuration $\{A, B\}$ is finite.

Recall that a family of edges of a bipartite graph is called\emph{edge covering} if each vertex is incident to some edge of this family. Note that this condition is equivalent to the surjectivity of the canonical projections, each of which maps the set of edges to one of two shares, matching each edge with a vertex incident to it from the considered share. Thus, in the notation of the proof of Theorem~\ref{thm:const_N_s}, the set $C\ss C_s$ is in the $s$ position if and only if $\mu_s^{- 1} (C)$ is an edge covering of the graph $G (A, B)$, so $N (A, B)$ is the number of distinct edge coverings of the graph $G (A, B)$.

\begin{prop}\label{prop:configuration_graph_realization}
Let $G=(V, E)$ be a finite bipartite graph with parts $V_1$ and $V_2$ having at least one edge cover. Then there exists a natural $n$ and such an embedding $\nu\: V\to\R^n$ such that $\bigl\{\nu (V_1),\nu (V_2)\bigr\}$ is the configuration , and the map $\nu$ generates an isomorphism of the graphs $G$ and $G\bigl (\nu (V_1),\nu (V_2)\bigr)$.
\end{prop}

\begin{proof}
Let $V_1=\{a_1,\ldots, a_p\}$, $V_2=\{b_1,\ldots, b_q\}$. Put $n=p+q$. Let $e_i$ denote the $i$th base vector of the standard basis in $\R^n$, and let $\nu (a_i)=e_i$.

For each $j\in\{1,\ldots, q\}$, we denote by $I_j$ the set of all $i$ such that $a_ib_j\in E$, and let $|I_j|$ be the number of elements in the set $I_j$. Put $N=1+\max_j|I_j|$, $m_j=N-|I_j|$ and for each $j\in\{1,\ldots, q\}$ let
$$
\nu (b_j)=\sqrt{m_j} e_{p+j}+\sum_{i\in I_j} e_i.
$$

If $a_ib_j\in E$, then $i\in I_j$ and, therefore, $\bigl|\nu (a_i)\nu (b_j)\bigr|^2=m_j+|I_j|-1=N-1$ . If $a_ib_j\not\in E$, then $i\not\in I_j$ and, therefore, $\bigl|\nu (a_i)\nu (b_j)\bigr|^2=m_j+|I_j|+1=N+1$. Since the graph $G$ has at least one edge covering, for each $a_i\in V_1$ and each $b_j\in V_2$ we have $\bigl|\nu (a_i)\nu (V_2)\bigr|=\bigl|\nu (b_j)\nu (V_1)\bigr|=\sqrt {N-1}$, so $\bigl\{\nu (V_1),\nu (V_2)\bigr\}$ is the final configuration. The fact that $\nu$ is an isomorphism of the graphs $G$ and $G\bigl (\nu (V_1),\nu (V_2)\bigr)$ is obvious from the construction.
\end{proof}

From the theorem~\ref{thm:19} and the sentence~\ref{prop:configuration_graph_realization} we instantly get the following result.

\begin{cor}
There is no bipartite graph having exactly $19$ or $37$ edge coverings.
\end{cor}

\begin{cor}
There is no configuration $\{A, B\}$ with $N (A, B)=19$ and $N (A, B)=37$ for finite subsets of $A$ and $B$ of a boundedly compact space with strictly internal metric.
\end{cor}

These studies were recently continued by Z.\, N.~Ovsyannikov~\cite{Ovs5}. He introduced the concept of an `` atomic bipartite graph'', determined the decomposition of an arbitrary bipartite into atomic graphs, and found out how the number of edge coverings of atomic graphs and the resulting bipartite are related. This allowed us to continue the sequence and show that the number of edge coverings of bipartite graphs, and hence the number of shortest arcs connecting a pair of compact sets, cannot be $41$, $59$ and $67$. In addition, Ovsyannikov found that in the range from $1$ to $1000$, all numbers except $19$, $37$, $41$, $59$, $67$, and also, possibly, except for $82$, $97$, $149$, $197$, $223$, $257$, $291$, and $379$ are realized as the number of edge coverings (shortest).

\begin{rk}
Thus, there is an interesting sequence of natural numbers, the initial segment of which has the form $19, 37, 41, 59, 67,\ldots,$. We checked this sequence on the well-known site {\tt https://oeis.org/}, which as of July 30, 2017 contained $289,946$ sequences. It turned out that this sequence is not there. It would be interesting to find the following members of this sequence.
\end{rk}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\renewcommand\bibname{Refenences to Chapter~\thechapter}
\addcontentsline{toc}{section}{\bibname}
\renewcommand{\refname}{\bibname}

\begin{thebibliography}{9}
\bibitem{Bogdewicz5} Bogdewicz A. ``Some Metric Properties of Hyperspaces''. Demonstratio Mathematica, 2000, v.~33, pp.~135-149.

\bibitem{Hosoya5} Hosoya H. ``Topological index. A newly proposed quantity characterizing the topological nature of structural isomers of saturated hydrocarbons''. Bulletin of the Chemical Society of Japan, 1971, v.~44 (9), pp.~2332–2339.

\bibitem{Gutman5} Gutman I. ``Polynomials in graph theory''. In: Bonchev D., Rouvray D.H., Chemical Graph Theory: Introduction and Fundamentals, Mathematical Chemistry 1, Taylor \& Francis, 1991, pp.~133–176.

\bibitem{Honigs5} Honigs K. ``Missing edge coverings of bipartite graphs and the geometry of the Hausdorff metric''. J. Geom., 2013, v.~104, pp.~107--125.


%l\bibitem{Ovs5} Овсянников З.Н.,  ``Количество реберных покрытий двудольных графов или кратчайших с фиксированнми концами в пространстве компактов в $\R^n$.'' Доклады Академии Наук, 2016, т.~466 (4), сс.~402--405.

\end{thebibliography}

\vfill\eject

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{\Huge Exercises to Chapter~\thechapter}
\markright{Exercises to Chapter~\thechapter.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{exe}
%Приведите пример метрического пространства $X$ и подмножеств $A,B\in\cH(X)$, для которых некоторое множество $C_s$ не лежит в $\cH(X)$. Приведите пример, в котором $C_s\in\cH(X)$, но $C_s$ не находится в $s$-положении между $A$ и $B$.
%\end{exe}



==> refs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addcontentsline{toc}{chapter}{\bibname}

\begin{thebibliography}{99}
\bibitem{blog} \url{http://mathoverflow.net/questions/212364/on-the-global-structure-of-the-gromov-}\\ \url{hausdorff-metric-space}
\bibitem{BurBurIva} D.\,Yu.~Burago, Yu.\,D.~Burago, S.\,V.~Ivanov, \emph{A Course in Metric Geometry}, AMS, Providence, RI, 2001.
\bibitem{IvaTuzLocalStrIsom} Ivanov A.O., Tuzhilin A.A. \emph{Local Structure of Gromov-Hausdorff Space near Finite Metric Spaces in General Position}, ArXiv e-prints, arXiv:1611.04484, 2016.
\bibitem{IvaNikolaevaTuz} Ivanov A.O., Nikolaeva N.K., Tuzhilin A.A. \emph{The Gromov-Hausdorff Metric on the Space of Compact Metric Spaces is Strictly Intrinsic}. ArXiv e-prints, arXiv:1504.03830, 2015.
\bibitem{Memoli} Chowdhury S., Memoli F. \emph{Constructing Geodesics on the Space of Compact Metric Spaces}. ArXiv e-prints, arXiv:1603.02385, 2016.
\bibitem{IvaIliadisTuz} Ivanov A.O., Iliadis S., Tuzhilin A.A. \emph{Realizations of Gromov-Hausdorff Distance}. ArXiv e-prints, arXiv:1603.08850, 2016.
\bibitem{IvaTuzIrreducible} Ivanov A.O., Tuzhilin A.A. \emph{Gromov--Hausdorff Distance, Irreducible Correspondences, Steiner Problem, and Minimal Fillings}. ArXiv e-prints, 1604.06116, 2016.
\bibitem{IvaTuzGeometryGHandSimplexes} Ivanov A.O., Tuzhilin A.A. \emph{Geometry of Compact Metric Space in Terms of Gromov-Hausdorff Distances to Regular Simplexes}. ArXiv e-prints, arXiv:1607.06655, 2016.
\bibitem{IvaTuzLocalStrEmbed} Ivanov A.O., Iliadis S., Tuzhilin A.A. \emph{Local Structure of Gromov-Hausdorff Space, and Isometric Embeddings of Finite Metric Spaces into this Space}. ArXiv e-prints, arXiv:1604.07615, 2016.
\bibitem{FFG} A.~Fomenko, D.~Fuchs \emph{Homotopical Toology}, Springer Publ., Switzerland, 2016.
\bibitem{John} John F. \emph{On quasi-isometric mappings, I}, Commun. Pure Appl. Math., 1968, v. 21, pp. 77--110.
\bibitem{MazurUlam} Mazur S., Ulam S. \emph{Sur les transformations isom\'etriques d’espaces vectoriels norm\'es}, C. R. Acad. Sci. Paris, 1932, v. 194, pp. 946--948.
    \end{thebibliography}

